Syntax-Aware Network for Handwritten Mathematical Expression Recognition

Handwritten mathematical expression recognition (HMER) is a challenging task that has many potential applications. Recent methods for HMER have achieved outstanding performance with an encoder-decoder architecture. However, these methods adhere to the paradigm that the prediction is made "from one character to another", which inevitably yields prediction errors due to the complicated structures of mathematical expressions or crabbed handwritings. In this paper, we propose a simple and efficient method for HMER, which is the first to incorporate syntax information into an encoder-decoder network. Specifically, we present a set of grammar rules for converting the LaTeX markup sequence of each expression into a parsing tree; then, we model the markup sequence prediction as a tree traverse process with a deep neural network. In this way, the proposed method can effectively describe the syntax context of expressions, alleviating the structure prediction errors of HMER. Experiments on three benchmark datasets demonstrate that our method achieves better recognition performance than prior arts. To further validate the effectiveness of our method, we create a large-scale dataset consisting of 100k handwritten mathematical expression images acquired from ten thousand writers. The source code, new dataset, and pre-trained models of this work will be publicly available.

==> latex/article/conclusion.tex <==
\section{Limitation}
As it is illustrated in Fig. \ref{Histograms}, distorted and sticking components of ME can cause failure to SAN prediction, which leads to the under/over translation. Fig. \ref{Histograms} gives four typical examples on CROHME (a and b) and HME100K (c and d) dataset.

\begin{figure}[h] 
    \centering
    \includegraphics[width=0.48\textwidth]{latex/images/bad_case.pdf}
    \caption{Limitation sample examples with the ground truth and recognition results of SAN. Characters in red color are mispredictions.} 
    \label{Histograms}
\end{figure}


\section{Conclusions}
%In this paper, we propose SAN, a new syntax-aware encoder-decoder model that incorporates syntax information into an encoder-decoder network for the first time. The model unifies grammatical structure with encoder-decoder in an end-to-end framework, improving recognition accuracy and reducing computation cost. Extensive experiments on two benchmarks datasets show the superior performance of our SAN than prior arts. Furthermore, we contribute a new HME100K dataset to the community. To the best of our knowledge, it is the first largest realistic scenario HMER dataset. In our future work, we shall explore an unsupervised technique to learn the SAN and enlarge the HME100K dataset.
%In this paper, we propose SAN, a new syntax-aware encoder-decoder model that incorporates syntax information into an encoder-decoder network for the first time.  The model unifies grammatical structure with encoder-decoder in an end-to-end framework, which improves the recognition accuracy and reduces the computation cost. Extensive experiments on two benchmarks datasets, CROHME2014, CHOHME2016 show the superior performance of our SAN than prior arts. Furthermore, we contribute a new HME100K dataset to the community. To the best of our knowledge, it is the first and the largest realistic scenario HMER dataset. We shall explore an unsupervised technique to learn the SAN and enlarge the HME100K dataset in our future work.
This paper has presented an unconventional method for handwritten mathematical expression recognition by combining syntax information and visual representations to make robust predictions. To our best knowledge, the proposed syntax-aware network is the first to effectively incorporate the grammar rules into deep feature learning. Our method not only predicts LaTeX markup results but also directly produces the tree structure output that can precisely describe the component relationship of mathematical expressions. Experiments on the benchmark datasets and the proposed HME100K dataset have validated the effectiveness and efficiency of our method. In our future work, we are interested in extending the proposed method to recognize other complicated structure objects.
%This paper has presented an unconventional method for handwritten mathematical expression recognition, making the predictions by combining syntax information and visual representations. To our best knowledge, the proposed syntax-aware network is the first time to incorporate the grammar rules into deep feature learning. Our method not only makes the prediction of LaTex markup results, but also directly produces the tree structure output that can precisely describe the component relationship of mathematical expressions. Experiments on the benchmark datasets and the proposed HME100k dataset have validated the effectiveness and efficiency of our method. In our future work, we are interested in extending the proposed method in recognizing other objects of complicated structure.

      

%This paper has presented a novel neural network architecture for robust and efficient mathematical expression recognition. The proposed syntax-aware network (SAN) introduces syntactic information into the deep network for the first time via incorporating grammar rules into feature learning. SAN can directly produce the tree structure output that fulfills the structural relationships besides generating latex output of mathematical expression. Experiments on the two CROHME benchmarks datasets and our HME100K dataset have demonstrated that our approach achieves significant improvements over state-of-the-arts. We assume that the proposed method is not only limited to mathematical expression recognition but also has the potential to be extended to object recognition and scene recognition tasks with complex structural relationships. In our future work, besides improving the performance and speed of the method, we will further try to apply it for tasks such as question answering based on HME images.

\section{Acknowledgement}

This work was supported by National Key R\&D Program of China, under Grant No. 2020AAA0104500 and National Natural Science Foundation of China 61733007.

==> latex/article/dataset.tex <==




\section{The HME100K Dataset}
%As shown in table \ref{statistics}, the HME100K dataset provides 99,110 images (74,502 for training and 24,607 for testing) with 247 kinds of symbol classes. The data size is increased tenfold compared to the CRHOME 2016 dataset. Instead of asking specific writers to create mathematical expressions (MEs), HME100K acquires the MEs from an Internet application. 
This section presents the new dataset HME100K, consisting of 74,502 images for training and 24,607 images for testing with 245 symbol classes, as shown in Table \ref{statistics}. Compared to CRHOME 2019\cite{mahdavi2019icdar} dataset, the data size is increased tenfold. The data were collected from tens of thousands of writers who wrote the MEs on papers and uploaded them to an internet application.   

As tens of thousands of writers participate in writing MEs, the variety of writing styles creates unique features to our MEs dataset.  Consequently, our dataset HME100K becomes more authentic and realistic with variations in color, blur, complicated background, twist, illumination, longer length, and complicated structure. Samples images from the dataset are shown in Fig. \ref{dataset}(b-h).
Furthermore, the maximum character length in HME100K is 184, which is almost twice longer than CROHME. HME100K also has a longer average sequence length than CROHME. For additional information about the HME100K dataset, please refer to the supplementary materials.

%Figure \ref{Histograms} shows the percentages of 20 most frequently observed symbols in HME100K and CROHME2016. 



% The CROHME competition datasets \cite{mouchere2014icfhr, mouchere2016icfhr2016} are the previous largest HMER datasets. 
% The images are generated from the online trajectories of handwritten mathematical expressions, results in simple and uniform background (Figure \ref{dataset}(a)).
% The CROHME 2014 dataset contains 8,836 training images and 986 testing images, and the CROHME 2016 dataset uses the same training set but adds additional 161 testing images. 
% The number of symbol class of CROHME 2014/2016 is 101. 
% The motivation for introducing the HME100K dataset is that the CROHME dataset is not large and diverse enough to objectively train and test the current deep learning based HMER models. 
% Actually, the tree-structured decoder \cite{zhang2020tree} outperforms DenseWAP \cite{wu2018image}  on the CROHME 2016 dataset, but the conclusion differs when pre-training them on the larger HME100K dataset (Table \ref{transfer learning}). 

\begin{figure}[h] 
    \centering
    \includegraphics[width=0.43\textwidth]{latex/images/dataset.pdf}
    \caption{Sample images from (a) the CROHME dataset and (b-h) the HME100K dataset.} 
    \label{dataset}
\end{figure}





==> latex/article/experiment.tex <==
\section{Experiments}
We evaluate our method performance on two CROHME benchmark datasets and the proposed HME100K and make the comparison with the state-of-the-art methods. 

\begin{table*}[htbp]
    \renewcommand\arraystretch{0.3}
    \centering
    \caption{Expression Recognition Rate (ExpRate) and Expression Structure Prediction Rate (ESPR) performance of our model and other state-of-the-art methods on CROHME 2014 and CROHME 2016. All results are reported as a percentage (\%). Our model achieves the best performance on all public datasets. $\star$ indicates the methods that used data augmentation during the training process.}
    \label{contrast results}
    \begin{tabular}{c|ccc|ccc|ccc}%l=left, r=right,c=center分别代表左对齐，右对齐和居中，字母的个数代表列数
    \toprule[1.5pt]
    \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{CROHME 2014}} & \multicolumn{3}{c|}{\textbf{CROHME 2016}} & \multicolumn{3}{c}{\textbf{CROHME 2019}} \\
    
     & \textbf{ExpRate}&\textbf{$\leq$1}&\textbf{$\leq$2}&\textbf{ExpRate}&\textbf{$\leq$1}&\textbf{$\leq$2}&\textbf{ExpRate}&\textbf{$\leq$1}&\textbf{$\leq$2}\\ \midrule[1pt]
    
    WYGIWYS \cite{deng2017image}&       36.4& -& -& -& -& -& -& -& -\\
    WAP \cite{zhang2017watch}&          40.4& 56.1& 59.9& 44.6& 57.1& 61.6& -& -& -\\
    PAL \cite{wu2018image}&             39.7& 56.8& 65.1& -& -& -& -& -& -\\
    PAL-v2 \cite{wu2020handwritten}&    48.9& 64.5& 69.8& 49.6& 64.1& 70.3& -& -& -\\
    PGS \cite{le2019pattern} & 48.8& 66.1& 73.9& 36.3& -& -& -& -& -\\
    TAP \cite{zhang2018track}& 48.5& 63.3& 67.3& 44.8& 59.7& 62.8& -& -& -\\
    DLA \cite{le2020recognizing}& 49.9& -& -& 47.3& -& -& -& -& -\\
    DWAP \cite{zhang2018multi}&     50.1& -& -& 47.5& -& -& -& -& -\\
    DWAP-MSA \cite{zhang2018multi}& 52.8& 68.1& 72.0& 50.1& 63.8& 67.4& 47.7& 59.5& 63.3\\
    DWAP-TD \cite{zhang2020tree}&   49.1& 64.2& 67.8& 48.5& 62.3& 65.3& 51.4& 66.1& 69.1\\
    WS-WAP \cite{truong2020improvement}& 53.7& -& -& 52.0& 64.3& 70.1& -& -& -\\
    MAN \cite{wang2019multi}& 54.1& 68.8& 72.2& 50.6& 64.8& 67.1& -& -& -\\
    RBR \cite{truong2020improvement}& 53.4& 65.2& 70.3& 52.1& 63.2& 69.4& 53.1& 63.9& 68.5 \\
    DWAP + CTC \cite{nguyen2021temporal}& 51.0& -& -& 50.0& -& -& -& -& -\\
    BTTR \cite{zhao2021handwritten}& 54.0& 66.0& 70.3& 52.3& 63.9& 68.6& 53.0& 66.0& 69.1 \\
    Li \emph{et al.} \cite{DBLP:conf/icfhr/LiJLZ20}$^\star$ & 56.6& 69.1& 75.3& 54.6& 69.3& 73.8& -& -& - \\
    Ding \emph{et al.} \cite{10.1007/978-3-030-86331-9_39}$^\star$ & 58.7& -& -& 57.7& 70.0& 76.4& 61.4& 75.2& 80.2 \\
    \textbf{SAN}&  \textbf{56.2}& \textbf{72.6}& \textbf{79.2}& \textbf{53.6}& \textbf{69.6}& \textbf{76.8}& \textbf{53.5}& \textbf{69.3}& \textbf{70.1}\\ 
    \textbf{SAN}$^\star$&  \textbf{63.1}& \textbf{75.8}& \textbf{82.0}& \textbf{61.5}& \textbf{73.3}& \textbf{81.4}& \textbf{62.1}& \textbf{74.5}& \textbf{81.0}\\ 
    \bottomrule[1.5pt]
    \end{tabular}
\end{table*}

% \begin{table*}[htbp]
%     \renewcommand\arraystretch{0.8}
%     \centering
%     \caption{Expression Recognition Rate (ExpRate) and Expression Structure Prediction Rate (ESPR) performance of our model and other state-of-the-art methods on CROHME 2014 and CROHME 2016. All results are reported as a percentage (\%). In every column, the best performance score is shown in bold font, and the second-best score is shown with an underline. Our model achieves the best performance on both public datasets. }
%     \label{contrast results}
%     \begin{tabular}{c|ccccc}%l=left, r=right,c=center分别代表左对齐，右对齐和居中，字母的个数代表列数
%     \toprule[1.5pt]
%     \textbf{Dataset} & \textbf{Model}&\textbf{ExpRate}&\textbf{$\leq$1}&\textbf{$\leq$2}&\textbf{ESPR}\\ \midrule[1pt]
%     \multirow{10}{*}{CROHME 2014} & UPV \cite{mouchere2014icfhr}&       37.2&   44.2&   47.3&   -\\
%                                  & TUAT \cite{mouchere2014icfhr}&      25.7&   33.2&   35.9&    -\\
%                                  & UNATES \cite{mouchere2014icfhr}&     26.1&   33.9&   38.5&    -\\
%                                  & WYGIWYS \cite{deng2017image}&       36.4&   -&   -&   -\\
%                                  & WAP \cite{zhang2017watch}&          40.4& 56.1& 59.9& -\\
%                                  & PAL \cite{wu2018image}&             39.7& 56.8& 65.1& -\\
%                                  & PAL-v2 \cite{wu2020handwritten}&    48.9& \underline{64.5}& \underline{69.8}& -\\
%                                  & DenseWAP \cite{zhang2018multi}&     43.0& 57.8& 61.9& 63.2\\
%                                  & DenseWAP-TD \cite{zhang2020tree}& \underline{49.1}& 64.2& 67.8& \underline{68.6} \\
%                                  & \textbf{SAN}&                \textbf{56.2}& \textbf{72.6}& \textbf{79.2}&\textbf{76.3}\\ \midrule[1pt]
%     \multirow{6}{*}{CROHME 2016} & TOKYO \cite{mouchere2016icfhr2016}&           43.9& 50.9& 53.7& 61.6\\
%                                 & WAP \cite{zhang2017watch}&           37.1& -& -& -\\
%                                  & PAL-v2 \cite{wu2020handwritten}&    \underline{49.6}& \underline{64.1}& \underline{70.3}& -\\
%                                  & DenseWAP \cite{zhang2018multi}&     40.1& 54.3& 57.8& 59.2\\
%                                  & DenseWAP-TD \cite{zhang2020tree}&   48.5& 62.3& 65.3& \underline{65.9}\\
%                                  & \textbf{SAN}             &  \textbf{53.6}& \textbf{69.6}& \textbf{76.8}&\textbf{73.0}\\  
%     \bottomrule[1.5pt]
%     \end{tabular}
% \end{table*}


% \begin{table}[h]
%     \renewcommand\arraystretch{0.4}
%     \centering
%     \caption{Statistics of HME100K testing set. The testing set is divided into 3 different subsets: \textbf{easy}, \textbf{moderate} and \textbf{hard}. The ExpRates on three HME100K subsets are tested by DenseWAP-TD and SAN. The last row shows the ExpRate gap between DenseWAP-TD and SAN}
%     \label{subset performance}
%     \begin{tabular}{c|cccc}%l=left, r=right,c=center分别代表左对齐，右对齐和居中，字母的个数代表列数
%     \toprule[1.5pt]
%     \textbf{HME100K}& \textbf{Easy}& \textbf{Moderate}& \textbf{Hard}&  \textbf{Hard} &\\\midrule[1pt]
%     Image size&       7721&   10445&   6435& 24607&\midrule[0.5pt]\\
%     DenseWAP-TD\cite{zhang2020tree}&    76.2&  63.2& 45.4& 62.6&-\midrule[0.5pt]\\
%     SAN&  79.2&  67.6& 51.5&-& \midrule[0.5pt]\\
%     gap&               3&   4.4&  6.1& -&-&
%     \bottomrule[1.5pt]
%     \end{tabular}
% \end{table} 

% \begin{table}[t]
%     \renewcommand\arraystretch{0.7}
%     \centering
%     \caption{Inference speed of DenseWAP-TD and SAN. ``FPS'' means frames per second.}
%     \label{inference speed}
%     \begin{tabular}{c|r}%l=left, r=right,c=center分别代表左对齐，右对齐和居中，字母的个数代表列数
%     \toprule[1.5pt]
%     \textbf{Model}&   \textbf{FPS}\\ \midrule[1pt]
%     DenseWAP-TD\cite{zhang2020tree}&      6.9 \\
%     \textbf{SAN}&    \textbf{23.9}\\ 
%     \bottomrule[1.5pt]
%     \end{tabular}
% \end{table}


\subsection{Datasets}
We use the Competition on Recognition of Online Handwritten Mathematical
Expressions (CROHME) benchmark, which currently is the most widely used public dataset for
handwritten mathematical expression to train and validate the HMER model. 
%Each ME in the CROHME dataset is saved in an InkML file, including handwritten stroke trajectory information and ground truth in MathML and LATEX formats.
We convert the handwritten stroke trajectory information in the InkML files into image format for the training and test sets. Sample of CROHME images is shown in (Fig. \ref{dataset}(a)). 

The CROHME training set consists of 8,836 expressions, including 101 math symbol classes, while the test set number of expressions are different according to the year they were published. 
We evaluate our model on CROHME 2014 test set\cite{mouchere2014icfhr}, CROHME 2016 test set \cite{mouchere2016icfhr2016} and CROHME 2019 test set \cite{mahdavi2019icdar} contain 986, 1147 and 1199 expressions respectively.


%\noindent\textbf{CROHME 2014 dataset} \cite{mouchere2014icfhr} 986 images for evaluation whereas \noindent\textbf{CROHME 2016 dataset} \cite{mouchere2016icfhr2016} consists of 1147 test set images. 

\subsection{Implementation Details}
The proposed model SAN is implemented in PyTorch.  All experiments are conducted on a single Nvidia Tesla V100 with 32GB RAM, and the batch size is set at 8.
The hidden state sizes of the two GRUs are set at 256. The dimensions of word embedding and relation embedding are set at 256. 
The Adadelta optimizer \cite{zeiler2012adadelta} is used during the training process, in which $\rho$ is set at 0.95 and $\epsilon$ is set at $10^{-6}$. 
The learning rate starts from 0 and monotonously increases to 1 at the end of the first epoch. 
After that the learning rate decays to 0 following the cosine schedules \cite{zhang2019bag}. 
% We train the model from scratch for 200 epochs on the CROHME2014/2016 datasets and only for 20 epochs on the HME100K dataset due to its large data size.   
Following most previous works, no data augmentation is applied during training for the fair comparisons. 
% As the image size of the HME100K dataset changes greatly, we normalize the image height to 120 pixels before training.

\subsection{Evaluation Protocol}
\noindent\textbf{Recognition Protocol.} Expression recognition rate (ExpRate) is the widely used recognition protocol for mathematical expression recognition, defined as the percentage of predicted mathematical expressions accurately matching the ground truth. ExpRate $\leq$ 1 and $\leq$ 2 indicate the expression recognition rates are tolerable at most one or two symbol-level errors.

\noindent\textbf{Structure Recognition Protocol.} Expression Structure Prediction Rate (ESPR) is used as the structure recognition protocol. ESPR is calculated by the percent of MEs whose structure is recognized correctly irrespective of symbol labels.

\subsection{Comparisons with State-of-the-arts}
In this subsection, we measure our proposed method on CROHME 2014, CROHME 2016 and CROHME 2019 datasets and compare the performance with other state-of-the-art methods. Most of the previous methods do not use data augmentation, so we mainly focus on the results produced without data
augmentation. Note that our method is not with the beam search process to obtain additional performance improvements.

\noindent\textbf{Evaluation on CROHME dataset}
As shown in table \ref{contrast results}, our method achieves state-of-the-art performance on all CROHME datasets. SAN outperforms MAN \cite{wang2019multi} by 3.1\%, BTTR \cite{zhao2021handwritten} by 1.3\% and BTTR \cite{zhao2021handwritten} by 0.5\% on CRHOME 2014, 2016 and 2019, respectively. In addition to ExpRate, SAN outperforms other state-of-the-art methods by a larger margin in ESPR. Thus, the SAN achievement demonstrates that incorporating syntax information into HMER neural network is effective and efficient.

\begin{table}[h]
    \renewcommand\arraystretch{0.1}
    \setlength\tabcolsep{2pt}
    \centering
    \caption{Performance of our model versus DWAP, DWAP-TD and BTTR on Easy (E.), Moderate (M.) and Hard (H.) HME100K test subsets. Inference speed reported as FPS means frames per second. The last column shows the parameter numbers of each model. The number in bold font corresponds to the best performance, and the second-best result is shown with an underline. Our model achieves the best performance on the HME100K dataset.}
    \label{subset performance}
    \begin{tabular}{c|cccccc}%l=left, r=right,c=center分别代表左对齐，右对齐和居中，字母的个数代表列数
    \toprule[1.5pt]
    \textbf{HME100K}& \textbf{E.}& \textbf{M.}& \textbf{H.}& \textbf{Total}& \textbf{FPS}& \textbf{P.N.} \\ \midrule[1pt]
    Image size&       7721&   10450&   6436& 24607& -&-\\\midrule[0.5pt]
    DWAP\cite{zhang2018multi}&    75.1&  62.2& 45.4& 61.9& \underline{23.3}& 4.8M\\
    DWAP-TD\cite{zhang2020tree}& 76.2& 63.2& 45.4& 62.6& 6.9 & 8.0M\\
    BTTR \cite{zhao2021handwritten}& \underline{77.6} & \underline{65.3} & \underline{46.0} & \underline{64.1} & 3.9 & 6.5M\\
    SAN&                      \textbf{79.2}&  \textbf{67.6}& \textbf{51.5}& \textbf{67.1}& \textbf{23.9} & 8.9M\\
    \bottomrule[1.5pt]
    \end{tabular}
\end{table}


\subsection{Evaluation on HME100K}

\noindent \textbf{Dataset Division.} For mathematical expressions, the structural complexity (S.C.) \cite{zhang2017tree} and character length (C.L.) significantly affect the model performance. With this in mind, we carefully allocate our test dataset into three subsets by difficulty. The allocation criteria is as follow:

$\begin{cases}
\textbf{Easy}, \qquad S.C. \in [0, 1] \ \& \ C.L. \in [1, 10) \\
\textbf{Moderate}, \ \ S.C. \in [0, 1] \ \& \ C.L. \in [10, 20) \\
\textbf{Hard}, \qquad otherwise
\end{cases}$

\noindent\textbf{Comparisons with previous methods.} In this subsection, we compare our proposed method with DWAP \cite{zhang2018multi}, DWAP-TD \cite{zhang2020tree} and BTTR \cite{zhao2021handwritten} on HME100K dataset. In order to be consistent with the reported inference process, DWAP-TD \cite{zhang2020tree} and BTTR \cite{zhao2021handwritten} use beam search, while DWAP \cite{zhang2018multi} doesn't. Specifically, as shown in table \ref{subset performance}, our method outperforms BTTR \cite{zhao2021handwritten} by 1.6\% on easy subset. However, as the difficulty of the test subset increases, the leading margin of our method increases to 5.5\% on the hard subset. The measurements of performances on different test subsets prove the superior robustness and structural awareness of our method.

In addition to the recognition accuracy, we evaluate the inference speed of our model against DWAP \cite{zhang2018multi}  and DWAP-TD \cite{zhang2020tree}  as summarised in table \ref{subset performance}. We measure the inference speeds in frame per second (FPS) on an HME100K test set via an Nvidia Tesla V100. Impressively, SAN is 3.5 times faster than DWAP-TD \cite{zhang2020tree}, while 2.6\% faster than DWAP \cite{zhang2018multi}, which indicates the efficiency of our method in minimizing computational costs.

\begin{table}[h]
    \renewcommand\arraystretch{0.3}
    \setlength\tabcolsep{3pt}
    \centering
    \caption{Ablation studies on CROHME datasets and HME100K datasets. The effect of recognition performance with regard to the two basic parameter settings: grammar syntax (G.S.) and syntax-aware attention (S.A. Attention). (\ding{51}) denotes the module existence while (\ding{53}) indicates the module absence.}
    \label{ablation studies}
    \begin{tabular}{c|ccccc}%l=left, r=right,c=center分别代表左对齐，右对齐和居中，字母的个数代表列数
    \toprule[1.5pt]
    \textbf{Model} & \textbf{G.S.} & \textbf{SA. Attention} & \textbf{ExpRate} & \textbf{Dataset} \\ \midrule[1pt]
    Baseline & \ding{53}&  \ding{53}& 49.1 &\multirow{3}{*} {\tabincell{c}{CROHME\\2014}}\\
    SAN\_GS  & \ding{51}&  \ding{53}& 55.3\\  
    SAN      & \ding{51}&  \ding{51}& 56.2\\ \midrule[1pt]
    
    Baseline & \ding{53}&  \ding{53}& 48.5 &\multirow{3}{*} {\tabincell{c}{CROHME\\2016}}\\
    SAN\_GS  & \ding{51}&  \ding{53}& 52.8\\  
    SAN      & \ding{51}&  \ding{51}& 53.6\\ \midrule[1pt]
    
    Baseline & \ding{53}&  \ding{53}& 51.4 &\multirow{3}{*} {\tabincell{c}{CROHME\\2019}}\\
    SAN\_GS  & \ding{51}&  \ding{53}& 53.0\\  
    SAN      & \ding{51}&  \ding{51}& 53.5\\ \midrule[1pt]
    
    Baseline & \ding{53}&  \ding{53}& 62.6 &\multirow{3}{*} {HME100K}\\
    SAN\_GS  & \ding{51}&  \ding{53}& 66.5\\  
    SAN      & \ding{51}&  \ding{51}& 67.1\\
    \bottomrule[1.5pt]
    \end{tabular}
\end{table}

\subsection{Ablation Study}
%In this section, we perform ablation studies to analyze the importance of different factors.
In this subsection, we perform ablation studies to analyze the impact of grammar syntax and syntax-aware attention modules. We trained all models from scratch and evaluated their performance on three datasets. SAN is the default model, while SAN-GS has the syntax-aware decoder but adopts coverage attention in the attention module instead of syntax-aware attention. The results are summarized in Table \ref{ablation studies}.
%To this end, we train multiple variations of our model with similar setting or configurations. 
%In the following experiments, all variations of our model are trained and evaluated on CROHME2014, CROHME2016 and HME100K dataset. The baselines shown in Table \ref{ablation studies} are provided by the state-of-the-art method tree-structured decoder.

\noindent \textbf{Impact of Grammar Syntaxes.} 
Table \ref{ablation studies} shows the integration of grammar syntaxes to baseline improves the recognition performance ExpRate by 6.2\% on CROHME 2014, 4.3\% on CROHME 2016, and 3.9\% on HME100K. Hence integrating grammatical constraints into the baseline model achieved improvements on all datasets, and this proofs the significance of grammar syntaxes incorporation to the decoder.   

\begin{figure}[h] 
    \centering
    \includegraphics[width=0.4\textwidth]{latex/images/sub_vs_coverage.pdf}
    \caption{Examples of (a) Converge-Attention and (b) Syntax-Aware Attention. The current recognized symbol is printed below each image. ``$E$'' indicates the non-terminal symbol (Eq.(1)). } 
    \label{grammar aware attention}
\end{figure}

\noindent \textbf{Impact of Syntax-Aware Attention.} As it is illustrated in Table \ref{ablation studies}, incorporating syntax-aware attention on top of grammar syntaxes increases the recognition performance rate ExpRate by 7.1\% on CROHME 2014, 5.1\% on CROHME 2016, and 4.5\% on HME100K from the baseline.  


%Furthermore, as shown in Fig \ref{grammar aware attention}, we compare the coverage attention and syntax-aware attention through a qualitative example. The images extracted from the prediction steps illustrate how the coverage-attention model disturbed by other sub-tree symbol while the syntax-aware attention model located the target symbol accurately. To clarify it further, using the coverage attention \cite{zhang2017watch}, the model wrongly focuses on the region of the symbol "1", predicting a redundant sub-tree that doesn't exist in the predicted position (Figure \ref{grammar aware attention}(a)).
%
Furthermore, as shown in Fig. \ref{grammar aware attention}, we compare the coverage attention and syntax-aware attention through a qualitative example. The images extracted from the prediction steps of coverage-attention and syntax-aware attention models illustrate how each model focuses on the target at each step.  As shown in (Fig. \ref{grammar aware attention}(a)), the coverage attention model wrongly focuses on the region of the symbol ``1", predicting a redundant sub-tree that doesn't exist in the predicted position. 
In contrast, the syntax-aware attentions model predicts an appropriate location that coincides with human intuitions (Fig. \ref{grammar aware attention}(b)).

    
% \subsection{Performance Evaluation on HME100K}

% In this section, we examine the performance of HMER models on the subsets of HME100k test sets labeled as easy, moderate, and hard. Moreover, we explore the advantage of pretraining on HME100k instead of starting from scratch.
    
% Table \ref{subset performance} summarizes the comparison of the performance of DenseWAP-TD and SAN on the three subsets of the HME100K test set. The results on three difficulty levels illustrate as the difficulty level increase, the performance gap between the two models increases. Accordingly, the superiority of SAN performance witnesses its ability to handle more complex MEs and the significance of integrating syntax components into HMER.    
    


==> latex/article/introduction.tex <==
\section{Introduction}

With the development of deep learning methods, the existing text recognition approaches are good at handling text lines in an image-to-sequence manner \cite{7801919, shi2018aster, shi2016robust, yang2019symmetry}. However, they may fail to deal with complicated structures such as mathematical expressions (ME). This paper investigates offline handwritten mathematical expression recognition (HMER), an important OCR task required by many applications like office automation, answer sheet correction, and assistance for visually disabled persons to understand mathematics. HMER is quite challenging, as a 2D structure relationship is essential for understanding mathematical expressions, which is seldom considered in previous deep learning-based methods. 
Besides, the ambiguities brought by handwritten input further increase the difficulty of HMER.

Early works have well studied ME's syntax structures, and the proper grammars are defined for HMER \cite{lavirotte1998mathematical, chan2001error, yamamoto2006line, alvaro2014recognition}. These grammars are only used for grouping the recognized symbols into a structural output, heavily relying on the performance of symbol recognition. Moreover, as these methods are mainly designed with handcraft features, their performance is far from the requirement of real-world applications.

Due to the recent advancement of deep neural networks, some recent studies \cite{deng2017image,zhang2017watch,zhang2018multi} handle HMER as an image-to-sequence prediction procedure using an encoder-decoder architecture, achieving significant performance improvements. However, these methods more or less neglect the syntax information contained in MEs.
To clearly illustrate this limitation, we take two recent network architectures as examples in Fig. \ref{architectures comparison}. Zhang \emph{et al.} \cite{zhang2017watch} propose the Watch, Attend and Parse (WAP) method that employs a fully convolutional network to encode handwritten images and a recurrent neural network as the string decoder to generate sequence outputs (Fig. \ref{architectures comparison}(a)). \cite{zhang2020tree} (DWAP-TD) attempt to consider the syntax information by decomposing the target syntactic structure tree into a sequence of sub-trees, where each sub-tree is composed of a parent node and a child node (Fig. \ref{architectures comparison}(b)). Though DWAP-TD can produce the output of a tree structure, it still follows the ``from one character to another'' paradigm that the next symbol prediction is mainly based on the current symbol. We argue that such methods don't explicitly consider the syntactic relationship of MEs in the learning process, which lacks the syntax constraints for generating a reasonable tree prediction.

\begin{figure}[h] 
    \centering
    \includegraphics[width=0.45\textwidth]{latex/images/Figure1.pdf}
    \caption{\textbf{Comparison of different architectures:} (a) An encoder-decoder framework WAP (b) A tree decoder DWAP-TD (c) Our model Syntax-Aware Network (SAN)}  
    \label{architectures comparison}
\end{figure}

To solve structure prediction error and improve the complex syntax tree understanding, we propose an elaborate grammar, which can naturally divide a syntax tree into different components and efficiently reduce tree structure ambiguity. Then, we establish an encoder-decoder network named syntax-aware network (SAN), which incorporates grammatical constraints and feature learning in a unified framework. Our intuition is that an ideal HMER model should parse handwritten mathematical expression images according to syntactic relationships, meanwhile effectively alleviating prediction errors caused by complex structures and crabbed writings. As shown in Fig. \ref{architectures comparison} (c), the prediction process of SAN follows the traverse process of a grammar tree, whose subtree is a significant component of a mathematical expression. In this manner, the syntactic relationship of adjacent components can be encoded in the proposed SAN model. Consequently, the prediction of SAN is made from one component to another component during the parsing procedure.
%For instance, as illustrated in Fig. \ref{bad cases}, SAN accurately predicts the given HMEs guided by syntax constraints. However, DenseWAP-TD fails to accurately predict due to a lack of syntax awareness.    

To evaluate the proposed SAN, we conduct the experiments on the two popular datasets, CROHME 2014\cite{mouchere2014icfhr} and CROHME 2016\cite{mouchere2016icfhr2016}. To further confirm the effectiveness of SAN, we collect and annotate a large-scale dataset for the evaluation, termed as HME100K. HME100K contains 100k handwritten mathematical expression images from ten thousand writers, mainly captured by cameras. Compared with the CHROME datasets\cite{mouchere2014icfhr,mouchere2016icfhr2016}, the data size of HME100K is increased tenfold. The results on CHROME 2014, CHROME 2016, and HME100K show that our method consistently achieves higher recognition rates over the state-of-the-art methods, demonstrating the advantage of  embedding syntax cues for HMER.


%We evaluated the performance of SAN on two benchmark datasets, CROHME2014, and CROHME2016. The results show that the proposed method achieves significantly higher recognition accuracies than the state-of-the-art performers, demonstrating that embedding of syntax cues is effectively integrated into a deep learning-based HMER system.     

 
%Compared with the previous benchmarks \cite{mouchere2014icfhr,mouchere2016icfhr2016}, the data size of HME100K is increased tenfold.




%propose a new handwritten mathematical expressions dataset, termed HME100K, which is the first dataset focus on real scene handwritten mathematical expressions. It contains 100K images from tens of thousands of writers. Compared with the previously largest CROHME dataset  \cite{mouchere2014icfhr,mouchere2016icfhr2016}, the data size is increased tenfold.

%Many applications in the field of education, \emph{e.g.} automatic homework searching and correcting, rely on the ability to convert scan or images of homework into editable and searchable data. 
%While modern Optical Character Recognition (OCR) systems are good at handling printed texts, HMER remains a critical yet under-addressed challenge in those systems because mathematical expressions usually have inherent grammatical structures and are presented in image with 2D spatial relations. 
%The ambiguities brought by handwritten input can further increase the difficulty of HMER. 



% HMER has been carried out in early works in separate steps. 
% The mathematical symbols are firstly segmented and recognized by classifiers such as support vector machines \cite{keshari2007hybrid} and hidden Markov models \cite{kosmala1999line};
% the 2D and syntactic structures of the expression are then parsed by
% manually defined grammars, \emph{e.g.} graph grammar \cite{lavirotte1998mathematical}, definite clause grammar \cite{chan2001error} and stochastic context-free grammar \cite{yamamoto2006line, alvaro2014recognition}.
% However, such manually defined grammars eventually result in cumbersome parsing rules, making HMER systems extremely sensitive to ambiguous inputs that are not avoidable in handwritten scenarios. 

 

%In early works, to well study the grammatical structures of MEs, manually defined grammars \cite{lavirotte1998mathematical, chan2001error, yamamoto2006line, alvaro2014recognition} are proposed. These grammars are only used in ME syntactic structure parsing step. They cannot guide the symbol segmentation and recognition steps. The limited feature learning ability of traditional method make HMER systems extremely sensitive to ambiguous inputs that are not avoidable in handwritten scenarios.



%Built upon the recent progress in sequence-to-sequence learning and neural networks \cite{sutskever2014sequence, chung2014empirical, huang2017densely}, some studies have addressed HMER with end-to-end trained encoder-decoder models and showed significant improvement in performance. 
%Zhang \emph{et al.} \cite{zhang2017watch} proposed a Watch, Attend and Parse (WAP) method that employs a fully convolutional network (FCN) to encode the handwritten image and a recurrent neural network as the string decoder to generate sequence outputs (Fig \ref{architectures comparison}.(a)).The next character prediction only depends on current step information, thus grammar is abandoned in WAP.
%A tree-structured decoder is proposed in \cite{zhang2020tree} by decomposing target syntactic structure tree into a sequence of sub-trees, where each sub-tree is composed of a parent node and a child node (Fig \ref{architectures comparison}.(b)).
%The tree-structured decoder outperforms string decoder in robustness because it constructs tree output that respects the structure of the expression.
%Nevertheless, the tree-structured decoder still adopts ``from one character to another'' paradigm makes it face the following challenges: 
%(1) Without grammatical constraint, complicated ME structure and crabbed handwriting easily cause relation prediction error.
%(2) It requires to predict two nodes (a parent node and a child node) for generating a new symbol, therefore this method is relatively slower than string decoder. %that predicts only once for generating each new symbol. 
%To alleviate structure prediction error and improve complicated syntax tree understanding, we propose an elaborate grammar, which can naturally divided a syntax tree into different components and efficiently reduces tree structure ambiguity. 
%We also propose an end-to-end trained model named Syntax-Aware Network (SAN), which incorporates grammatical constraints and feature learning in a unified framework. SAN reduces the structure prediction error of tree-structured decoder \cite{zhang2020tree} but obtains comparable inference speed with DenseWAP \cite{zhang2018multi}. 

%Meanwhile, we propose a new handwritten mathematical expressions dataset, termed HME100K, which is the first dataset focus on real scene handwritten mathematical expressions. It contains 100K images from tens of thousands of writers. Compared with the previously largest CROHME dataset  \cite{mouchere2014icfhr,mouchere2016icfhr2016}, the data size is increased tenfold.
%and the writer number is increased hundredfold in HME100K.

%The contribution of this paper is fourfold.
%First, the main contribution of this paper is the proposed syntax-aware network, which effectively embeds syntactic information into deep neural networks for the first time. Second, our method is an end-to-end trainable network that not only can predict the latex sequence but also generate the reasonable tree-structured output of formulas according to syntactic rules. Third, the experimental results on both the standard dataset and our dataset show our model improves the recognition significantly and 3.47 times faster inference time, compared to the tree-structured state-of-the-art HMER model \cite{zhang2020tree}.  This rapid inference time makes our model scalable to larger datasets.Fourth, we contribute a new large and diverse dataset to train the HMER models named HME100K to the community
The main contribution of this paper is the proposed syntax-aware network, which effectively embeds syntactic information into deep neural networks at the first time. 
Another contribution of this paper is the proposed large and diverse dataset HME100K. Compared with the existing benchmark datasets, our dataset includes the HME with longer lengths and more complicated structures, making it useful to promote more robust algorithms toward real-world applications.


\begin{figure}[tp] 
    \centering
    \includegraphics[width=0.45\textwidth]{latex/images/bad_cases_1.pdf}
    \caption{Sample Recognition Results of SAN and DWAP-TD. The SAN heatmaps indicate the model is focused on different components. The characters in red refer to the lost component during the prediction.}
    \label{bad cases}
\end{figure}
%First, from a theoretical point of view, this paper introduces SAN to the domain of HMER, which incorporates grammatical constraints into feature learning for the first time.
%Second, from a more applied point of view, this paper takes a step forward in HMER by extending state-of-the-art models \cite{zhang2020tree} with more accurate recognition and faster inference time.
%Third, we contribute a new large and diverse dataset to train the HMER models named HME100K to the community.
%This new dataset paves the way to train the HMER models with large and diverse enough data and to evaluate the performance of models objectively in a realistic scenario.



==> latex/article/methodology.tex <==


\section{ Syntax-Aware Network}

Formally, a SAN can be defined as a 7-tuple $G=(N, \Sigma, R, S, \Gamma, C, D)$, consisting of a finite set of non-terminal symbols ($N$), a finite set of terminal symbols ($\Sigma$), a finite set of production rules ($R$), a start symbol ($S$), a finite set of relations ($\Gamma$), an encoder ($C$) and a decoder ($D$). We design the grammar rules with two constraints: 1) It follows the standard reading orders: left-to-right, top-to-down. 2) The spatial relations between adjacent symbols are used. For a pair of adjacent symbols of HME, there are nine possible relations in total (left, right, above, below, low left, low right, upper left, upper right, inside). Due to constraint 1), we have removed ``left'' and ``low left'', and the rest 7 relations have been sustained to deal with all the cases of MEs in our implementation. Even though a ME may correspond to different LaTeX sequences, the syntax trees generated by our grammar rules are the same due to the two constraints.
% {\color{blue} We design the grammar rules with two constraints: 1) It follows common reading orders: left-to-right, top-to- down. 2) The spatial relation between adjacent symbols are used. Given a pair of adjacent symbols, there are 9 relations in total (left, right, above, below, low left, low right, upper left, upper right, inside). Due to constraint 1), for simplicity, ``left'', ``low left'' are removed, and 7 relations are remained that is able to cover all the cases of MEs with our implementation. Though a ME may correspond to different \LaTex sequences, whose syntax trees obtained by our grammar rules are the same due to the two constraints. This is a very good property for representing a ME. Besides, as relations are included by a syntax tree, which are more informative for HMER. }

The SAN transforms an image into a parse tree, of which the leaf nodes are terminal symbols or relations, and others are non-terminal symbols. There are two non-terminal symbols $S$ and $E$, where $S$ is the start symbol and servers as the tree's root. The terminal set $\Sigma$ contains all symbols that might be used in a LaTeX expression sequence.

The $R$ production rule can be used to construct the parse tree. The production rules are with the form of $\alpha\rightarrow\beta$, where $\alpha\in N$, $\beta \in (\Gamma \cup N \cup \Sigma) ^ *$ and the asterisk represents the Kleene star operation. Hence, a parent node ($\alpha$) can be split into a list of children nodes ($\beta$) containing terminal symbols, non-terminal symbols and relations.

$R$ has two production rules.
The first rule is an $S$ produce 1) an arbitrary terminal symbol followed by an $S$ on the right, 2) an $E$ or, 3) an empty string indicated by $\epsilon$:
\begin{equation}
    S\rightarrow\sigma S | E | \epsilon,
\end{equation}
where $\sigma\in\Sigma$ is an arbitrary terminal symbol and ``$|$'' separates alternatives. 
The second rule is an $E$ produces a string for each type of relation and then concatenates them. 
The string can be the relation followed by an S, or an empty string:
\begin{equation}
    E\rightarrow [((\gamma_1) S|\epsilon),\dots,((\gamma_7) S|\epsilon)],
    \label{node E}
\end{equation}
where $\gamma_i \in \Gamma$ is the $i^{th}$ type of relation in $\Gamma$, and [$\cdot$] is the concatenation operator. 

Fig. \ref{parsing procedure} illustrates the possible parsing procedure of an expression with the production rules.
To understand those rules intuitively, regard $S$ as an expression and $E$ an extendable structure. Assume that an expression may contain multiple extendable structures, whereas each extendable structure can be extended to multiple expressions with spatial relations. Moreover, the production rule is associated with a probability conditioned on the input image and the context state of the parent node.
Specifically, the conditional probability is defined as
\begin{equation}
p(\alpha\rightarrow\beta|c(\alpha),X) = D_{\alpha\rightarrow\beta}(c(\alpha),E(X)),
\end{equation}
where $X$ is the input image, $E(X)$ is the output of encoder, $c(\alpha)$ is the context state of $\alpha$ (will be detailed in Sec. 3.2) and $D_{\alpha\rightarrow\beta}(\cdot)$ is the output of decoder that corresponds to the production rule.

%Given the SAN parameters, an input image, and the inference procedure is described in Algorithm \ref{algorithm}. 
As illustrated in Algorithm \ref{algorithm}, given the SAN parameters and an input image, a tree traverse is implemented with a stack. Specifically, the implemented stack can guarantee the training process according to the traversal order on a syntax tree. Similarly, the prediction process is also implemented by stacking step by step.
The encoder takes an input image and down-samples it. Then based on the grammar rules, identify an expression and its extendable structures; meanwhile, the decoder calculates and selects the production rule with the highest probability. Consequently, generate new expressions with extendable structures and update the parse tree of the image in the LaTeX sequence.  
Once the parse tree is found, the recognition result can be acquired by traversing the tree in preorder. 
The remaining parts of this section focus on encoder, decoder, attention mechanism, and parameter learning. 

\begin{algorithm} 
    \setstretch{0.8}
    \caption{Inference process of SAN} 
    \label{algorithm}
    {\bf Input:} SAN parameters; The input image\\
    {\bf Output:} The parse tree of the image\\
    Encode the image\\
    Push $S$ and its context state onto the top of the stack
    \begin{algorithmic}
        \While{the stack is not empty} 
        {\\
            {\bf 1. }Pop a non-terminal symbol or relation together with its context state from the top of the stack\\
            {\bf 2.} Use  the  decoder  to  calculate  the  conditional probabilities of the production rules\\
            {\bf 3.} Select the production rule with the highest conditional probability\\
            {\bf 4.} Push each newly produced non-terminal symbol or relation in the rule with the context state onto the top of the stack\\
            {\bf 5.} Update the parse tree with the selected production rule
        }
        \EndWhile
    \end{algorithmic}
{\bf return} the parse tree
\end{algorithm}


% \begin{algorithm} 
% \setstretch{0.5}
% \caption{Inference process of SAN} 
% \label{algorithm}
% \KwIn{SAN parameters; The input image} 
% \KwOut{The parse tree of the image}
% \State Encode the image
% \State Push $S$ and its context state onto the top of the stack
% \State\While{the stack is not empty} 
% { 
%     \State Pop a non-terminal symbol or relation together with its context state from the top of the stack
%     \State Use  the  decoder  to  calculate  the  conditional probabilities of the production rules
%     \State Select the production rule with the highest conditional probability
%     \State Push each newly produced non-terminal symbol or relation in the rule with the context state onto the top of the stack
%     \State Update the parse tree with the selected production rule
% } 
% \State \Return the parse tree
% \end{algorithm}

\subsection{Encoder}
We use the densely connected convolutional network (DenseNet) \cite{huang2017densely} as the encoder. The DenseNet is an FCN that connects all networks in a feed-forward style and reinforces feature propagation and reuse by guaranteeing maximum information flow between layers in the network. Consequently, the FCN can handle an image of arbitrary size, making it appropriate for HMER since the sizes of handwritten images are usually in random sizes.
 
As a result, the encoder takes a gray-scale image $X$, with size of $1\times H\times W$, where $H$ and $W$ are height and width respectively, and returns a $C\times H/\zeta \times W/\zeta$ matrix, where $C$ is the channel number and $\zeta$ is the down-sampling factor.
Then the encoding is represented as $E(X) = [e_1,\ldots,e_L]$, where $L = H/\zeta \times W/\zeta$ and $e_i\in \mathbb{R}^C$.
Each element of $E(X)$ is related to a local region of the image.  
In our implementation, $C$ is set as 684 and $\zeta$ is set as 16.

\begin{figure}[h] 
\centering
\includegraphics[width=0.42\textwidth]{latex/images/decoder.pdf}
\caption{Syntax-Aware Decoder: Consisting of   GRU-$\alpha$, GRU-$\beta$, and the Syntax-Aware Attention Module. }
\label{decoder}
\end{figure}
\vspace{-0.3cm}

\subsection{Syntax-Aware Decoder}
As illustrated in Fig. \ref{decoder}, the decoder mainly consists of two Gated Recurrent Units (GRU) cells \cite{chung2014empirical} (indicated by GRU-$\alpha$, GRU-$\beta$) and a syntax-aware attention module.
Given the context state of a non-terminal symbol $\alpha$ and the encoding vector $E(X)$, the decoder returns the probability of each production rule that begins with $\alpha$.

We use a historical state and a partner state to describe the context state of the current parsing non-terminal symbol. 
The historical state $c_h^{\alpha}$ is used to keep track of the information of how the non-terminal symbol $\alpha$ is produced.
In addition, the word embedding of the latest generated terminal symbol or relation is used as the partner state $c_p^{\alpha}$ of the non-terminal symbol to capture the short-term contextual information. 
The first GRU-$\alpha$ takes $c_p^{\alpha}$ as the input vector and  $c_h^{\alpha}$ as the hidden vector, and outputs a new hidden vector $c_o^{\alpha}$:
\begin{equation}
    c_{o}^{\alpha} = \mathrm{GRU}(c_{p}^{\alpha}, c_{h}^{\alpha}).
\end{equation}
Then the attention module calculates a compact visual feature
\begin{equation}
\Omega =  \mathrm{Att}(E(X),c_{o}^{\alpha},att_{\alpha}(X)),
\end{equation}
where $\mathrm{Att}(\cdot)$ is the attention function and 
$att_{\alpha}(X)$ is the syntax-aware attention vector
which is detailed in Sec 3.3. 
The second GRU-$\beta$ takes $\Omega$ as the input vector and $c_o^{\alpha}$ as the hidden vector, and outputs a new hidden vector $c_\beta^{\alpha}$:
\begin{equation}
    c_\beta^{\alpha} = \mathrm{GRU}(\Omega,c_{o}^{\alpha}).
\end{equation}
We then aggregate $c_p^{\alpha}$, $c_\beta^{\alpha}$ and $\Omega$ to predict two branches of probabilities:
\begin{equation}
    \begin{split}
        p_{symbol}(\alpha\rightarrow\beta|c(\alpha),X) = \hspace{0.9in}\\
        \mathrm{softmax}(W_{s}(W_{p}c_p^{\alpha}
        + W_{g}c_\beta^{\alpha} + W_{t}\Omega))
    \end{split}
\end{equation}
\vspace{-0.5cm}
\begin{equation}
    \begin{split}
        p_{relation}(\alpha\rightarrow\beta|c(\alpha),X) = \hspace{0.9in} \\ \mathrm{sigmoid}(W_{r}(W_{p}c_p^{\alpha}
        + W_{g}c_\beta^{\alpha} + W_{t}\Omega))
    \end{split}
\end{equation}
where $W_s$, $W_p$, $W_g$, $W_t$ and $W_r$ are learnable parameters. 
$p_{symbol}(\alpha\rightarrow\beta|c(\alpha),X)$ is a probability vector with $|\Sigma| + 2$ dimensions. Note that there are three scenarios 1) $|\Sigma|$ dimensions for predicting terminal symbols, 2) one dimension for predicting $E$, and 3) one dimension for predicting an empty string.
For the first scenario, if the prediction of a terminal symbol ($\sigma$) has the highest probability, then apply the rule of $S\rightarrow \sigma S$ to update the parse tree, use the word embedding of $\sigma$ as the partner state of the newly generated $S$, and $c_\beta^{\alpha}$ as its historical state.
For the second scenario, if the prediction of $E$ has the highest probability, then apply $p_{relation}(\alpha\rightarrow\beta|c(\alpha),X)$ to predict the probability of each relation.
The relations with probabilities higher than 0.5 are sustained, and others are thrown away. 
For each remaining relation, we use the embedding of the relationship as the partner state of the following $S$, and use $c_\beta^{\alpha}$ as the historical state. Moreover, there is no need to consider parsing an $E$, because it has already been acquired from the relation branch.
For the third scenario, 
if the empty string has the highest probability, we update the parse tree with the rule of $S\rightarrow \epsilon$.


\subsection{Syntax-Aware Attention Module}
Instead of using the entire image feature for decoding, the attention module calculates a compact visual feature with the attention mechanism. 
We first compute a normalized weight for each local region of the image, and then use the weighted average to aggregate the local features.
We use the image encoding $E(X)$, the hidden state $c_o^{\alpha}$ and a syntax-aware attention vector $att_{\alpha}(X)$ to calculate the normalized weight vector:
\begin{equation}
\begin{split}
        \xi_\alpha = \mathrm{softmax}(W_{w}( \mathrm{tanh}(W_{o}c_{o}^{\alpha} +  \\ W_{\alpha}att_{\alpha}(X) + W_{e}E(x)))),
\end{split}
\end{equation}
where $W_w$, $W_o$, $W_{\alpha}$ and $W_e$ are learnable parameters, and $\xi_\alpha$ is a vector of length $L$. 
The compact visual feature 
\begin{equation}
\mathrm{Att}(E(X),c_{o}^{\alpha},att_{\alpha}(X)) = E(X)\xi_\alpha
\end{equation}
is computed by the matrix product. 
%A coverage vector based on the sumof all past attention probabilities is used in  \cite{zhang2017watch,zhang2020tree} to indicate whether a local region of the image has been parsed.
%We argue that, however, there is no need to keep track of all past attention probabilities in the SAN. 
Unlike \cite{zhang2017watch,zhang2020tree}, which used a coverage vector based on the sum of all past attention probabilities, SAN does not keep track of all past attention probabilities.
The attention drift problem happens because the attention probabilities of the numerator give no information for parsing the denominator but appear as the noise.  
Instead, we sum up the past attention probabilities along the path from the root of the parse tree to the current parsing node but not all past attention probabilities.
Therefore, we calculate the syntax-aware attention vector as follows:
\begin{equation}
att_{\alpha}(X) = \sum_i \xi_i, \hspace{0.1in} i\in path_{\alpha}.
\end{equation}

The syntax-aware attention vector can be efficiently traced by storing it as intermediate information with the stack. 

An attention self-regularization strategy is used to correct the attention. We use an additional reversed decoder to predict the parent node of each given child node.
The reversed decoder shares the same structure with the original one but operates the data in reverse. 
Thus we have two normalized weight vectors for predicting each non-terminal node $\beta$, the forward $\xi_\alpha$ and the reversed $\hat{\xi_\eta}$, where $\alpha$ is the parent of $\beta$ and $\beta$ is the parent of $\eta$.
We use a Kullback-Leibler (KL) divergence to regularize them
\begin{equation}
     \mathcal{L}_{reg} = -\sum \limits_\beta  \hat{\xi_\eta} \log \frac{\hat{\xi_\eta}}{\xi_\alpha}.
\end{equation}
The reversed decoder is jointly trained with SAN but is omitted during inference to skip additional inference time.

\begin{table*}[htp]
    \renewcommand\arraystretch{0}
    \centering
    \caption{Statistical comparison of the HME100K and CROHME2019 dataset. ``Max Length'' and ``Avg Length'' mean the maximum length and average length of the mathematical expression.}
    \label{statistics}
    \begin{tabular}{c|cccccc}%l=left, r=right,c=center分别代表左对齐，右对齐和居中，字母的个数代表列数
    \toprule[1.5pt]
    \textbf{Dataset}             & \textbf{Train Size}& \textbf{Test Size}&  \textbf{Symbol Class No.} & \textbf{Max Length} & \textbf{Avg Length} & \textbf{Writer No.} \\ \midrule[1pt]
    HME100K     & 74,502 & 24,607& 245 & 184 & 17.62 & $\thicksim$10K \\ \midrule[1pt]
    CROHME2019 & 8,836 & 1,199& 101 & 96 & 15.79 & $\thicksim$100 \\
    \bottomrule[1.5pt]
    \end{tabular}
\end{table*}

\subsection{Parameter Learning}
SAN is trained end-to-end under a multi-task setting, that aims to minimize the sum of symbol loss ($\mathcal{L}_{symbol}$), relation loss ($\mathcal{L}_{relation}$), reversed symbol loss ($\mathcal{L}_{symbol}^{rev}$) and attention self-regularization loss ($\mathcal{L}_{reg}$).

We use the teacher forcing strategy for accelerating convergence. The ground-truth parse tree is obtained for each training image by parsing the LaTeX sequence with the depth-first-search algorithm.  Thus, a list of parent-children samples is acquired from the parse tree. Afterward, deal with each sample sequentially according to the preorder of the tree until the entire tree is processed. Likewise, we use the reversed decoder to predict the parent node of each given child node. 
%We then use the ground-truth labels to calculate the symbol, reversed symbol and relation losses. 
Then using the ground-truth labels, we calculate the symbol, reversed symbol and the relation losses.
The attention self-regularization loss can be calculated by (12). Thus we can optimize the parameters by minimizing the following objective function with backpropgation
\begin{equation}
    \mathcal{L} = \mathcal{L}_{symbol} + \mathcal{L}_{relation} + \mathcal{L}_{symbol}^{rev} + \mathcal{L}_{reg}.
\end{equation}

    


==> latex/article/related_work.tex <==
\section{Related Work}
%HMER is a fundamental OCR task, which has attracted research interests in the past several decades. 
%In this section, we briefly introduce previous related works on HMER.
HMER is a critical branches of document analysis and recognition that can be applied to recognize answer sheets of mathematics and digitize numerous kinds of scientific literature.
Compared with conventional handwriting text recognition, HMER is a more challenging task due to ambiguities coming from handwriting style, the two-dimensional structures complexity, and irregular scales of handwritten mathematics symbols. 
Therefore, HMER can be divided into three major challenging tasks\cite{chan2000mathematical,mouchere2016advancing, zanibbi2012recognition}: grouping strokes of the same symbol by segmentation, recognizing the symbols, and grammar-guided symbols structural relationship analysis to generate a mathematical expression. Traditional HMER methods tried to solve these challenges sequentially and globally.  
%Traditional methods on HMER could be mainly separated into two steps: a symbol segmentation/recognition step and a grammar guided structure analysis step. 

%In the first step,several classic classification techniques were studied, such as HMM \cite{winkler1996hmm, kosmala1999line, hu2011hmm, alvaro2014recognition}, Elastic Matching \cite{chan1998elastic, vuong2010towards}, Support Vector Machines \cite{keshari2007hybrid}, etc.

The sequential methods\cite{chan2000mathematical,zanibbi2002recognizing,winkler1996hmm, kosmala1999line, hu2011hmm, alvaro2014recognition,chan1998elastic, vuong2010towards,keshari2007hybrid } first segment input expression into mathematical symbols, classify each symbol separately, and then the structural relationship analysis recognize the mathematical expression. These methods employed classification techniques such as HMM \cite{winkler1996hmm, kosmala1999line, hu2011hmm, alvaro2014recognition}, Elastic Matching \cite{chan1998elastic, vuong2010towards}, Support Vector Machines \cite{keshari2007hybrid}, and tree transformations\cite{zanibbi2002recognizing}. 
%In the second step, formal grammars were designed to model the 2D and syntactic structures of expression. 
%Lavirotte \emph{et al.} \cite{lavirotte1998mathematical} proposed to use graph grammar to recognize mathematical expression. 
%Chan \emph{et al.} \cite{chan2001error} incorporated correction mechanism into parser based on definite clause grammar (DCG). Yamamoto \emph{et al.} \cite{yamamoto2006line} modeled handwritten mathematical expressions with a stochastic context-free grammar and solved the recognition problem by using the CYK algorithm. 
On the other hand, the global approaches\cite{awal2014global, le2016system,alvaro2016integrated} apply a comprehensive strategy to learn mathematical symbols and their structural relationship analysis, while segmenting the symbols implicitly.
%
These methods handle HMER as a global optimization of mathematical expression segmentation, symbol recognition, and structure of the expression identification based on the symbol recognition results.
%In contrast to those traditional methods, our model incorporates grammatical structure and automatically learned encoder-decoder, therefore preventing from designing cumbersome rules. 

\begin{figure*}[h] 
\centering
\includegraphics[width=0.95\textwidth]{latex/images/parsing.pdf}
\caption{(a) A possible parsing procedure of $\sum\limits_ {i}^{n}a$ and (b) the parse tree. In the figure, the strings refer to non-terminal symbols in blue, terminal symbols in red, relations in yellow, and empty in grey.}
\label{parsing procedure}
\end{figure*}

%In recent years, deep learning gained prominence, and its techniques rapidly boosted the performance of HEMR. 
Recent deep learning-based HMER methods can be roughly classified into the sequence-to-sequence approach and the tree-structure approach. Most HMER methods extensively adopt the sequence-to-sequence approach.
%Most HMER methods extensively adopted encoder-decoder approaches based on attention. 
%The mainstream framework was encoder-decoder networks. 
The authors in\cite{deng2017image, zhang2018multi,zhang2017watch, zhang2018track, zhao2021handwritten, wang2019multi, truong2020improvement, nguyen2021temporal, le2020recognizing, zhang2018track, le2019pattern}  proposed an attention-based sequence-to-sequence model to convert the handwritten mathematical expression images into representational markup language LaTeX. Recently, Wu \emph{et al.}\cite{wu2021graph} designed a graph-to-graph(G2G) model that explores the HMEs structural relationship of the input formula and output markup, which significantly improve the performance.
%Similarly,
%Zhang \emph{et al.} \cite{zhang2017watch, zhang2018track } presented an end-to-end trainable network based on a sequence-to-sequence attention mechanism to recognize offline and online HMEs in a two-dimensional layout and produces a one-dimensional LaTeX markup.
%Zhang \emph{et al.} \cite{zhang2017watch} presented presented WAP (Watch, Attend and Parse), an end-to-end trainable network based on a sequence-to-sequence attention mechanism to recognize HMEs in a two-dimensional layout and produces a one-dimensional LaTeX markup.
%Zhang \emph{et al.} \cite{zhang2018track} proposed a sequence-to-sequence attention mechanism that encodes online handwritten mathematical expression images and decodes them into LaTeX markup.
The sequence-to-sequence approach improved the HMER performance. However, it lacks syntactic relationship awareness due to its inherited 1D nature, which causes inevitable prediction errors when dealing with 2D HMEs. 
% {\color{blue} Wu \emph{et al.}\cite{wu2021graph} use online information and convert the HMER as a graph-to-graph(G2G) learning task, which significantly improve the performance}.
%Wu \emph{et al.} \cite{wu2018image, wu2020handwritten} focused on the pair-wise adversarial learning strategy to improve the recognition accuracy.
%To alleviate the challenge of lack of data, Le \emph{et al.} \cite{le2019pattern} and Li \emph{et al.} \cite{li2020improving} employed distortion, decomposition and scale augmentation techniques, which achieved significant performance promotion. 
%Le \cite{le2020recognizing} proposed a dual loss attention model, which contains a new context match loss. Context matching loss is adapted to constrain the intra-class distance and enhance the discriminative power of model.
%The work \cite{DBLP:journals/corr/abs-2105-02412} proposed a transformer-based decoder and a novel training strategy that fully exploit the potential of the transformer in bidirectional language modeling.
%Recent studies \cite{shi2018tree, williams2018latent, choi2018learning, jacob-etal-2018-learning, shen2017neural, kuncoro-etal-2018-lstms} in natural language processing have paid attentions to using the tree structures to form better representations of natural language sentences. And recurrent neural networks (RNNs) also exhibit ability to implicitly encode the tree structure of natural language to implement syntactic processing mechanisms \cite{gulordava2018colorless, kuncoro-etal-2018-lstms, lakretz2019emergence}. Similar to natural language, MEs have a sequential overt form in LaTeX format, but the underlying structure of MEs is tree-like: smaller units (e.g., characters) are nested within larger units (e.g., component). However, most of previous studies adopt string decoder to generate sequence output, which ignore the implicit grammar syntaxes.

The tree-structure approach employs a tree-structured decoder to model the parent-child relationship of mathematical expression trees explicitly.
To recognize online HME, Zhang \emph{et al.} \cite{zhang2017tree} proposed tree-structured based on BLSTM, while Zhang \emph{et al.} \cite{zhang2020srd} proposed tree-structured based on sequential relation decoder (SRD).  
%Zhang \emph{et al.} \cite{zhang2017tree} proposed a tree-structured approach for online HMER based on BLSTM architecture with a unique trainable system that directly produces a stroke label graph labeling a mathematical expression.
%Similarly, in \cite{zhang2020srd}, a tree-structured approach based on sequential relation decoder (SRD) was proposed to decode expressions into tree structures for online handwritten mathematical expression recognition. 
%Zhang \emph{et al.} \cite{zhang2020tree} devised a tree-structured decoder to parse mathematical expression. At each step, a parent and child node pair was generated and the relation between parent node and child node reflects the structure type.
%On the other hand, to recognize offline HEMs, Zhang \emph{et al.} \cite{zhang2020tree} devised a tree-structured decoder that respects the parent-child relationship of trees during decoding until the final output tree.
On the other hand, to recognize offline HEMs, Zhang \emph{et al.} \cite{zhang2020tree} proposed a tree-structured decoder that attempts to consider the grammatical information by decomposing the target syntactic structure tree into a sub-tree sequence, where each sub-tree has a parent-child relationship.
%Contrast experiments proved tree-structured decoder exhibits better robustness than string decoder. Nevertheless, the tree-structured decoder still faces the following challenges: (1) Lack of grammatical constraints can cause irremediable structure prediction error. (2) It requires to predict two nodes (a parent node and a child node) for generating a new symbol, therefore this method is relatively slower than string decoder.
Generally, a tree-structured decoder exhibits better robustness compared to a string decoder. However, the existing tree-structured decoders have two limitations. 1) The lack of holistic representation of grammatical information in deep network feature learning. 
2) The methods theoretically attempt to consider the syntactic information; however, they couldn't escape from the vicious circle of the sequence-to-sequence string decoding scheme in practice.    

The difficulty of HMER mostly relies on considering syntactic relationship complexity rather than symbol recognition. Thus, we proposed a novel neural network architecture equipped with grammar rules that efficiently divides a syntax tree into different components to alleviate errors caused by tree structure ambiguity.
%
The proposed method learns the grammatical relationship between the structures based on the grammar rules and navigates the syntax tree to create components according to the structural relationship. The key differences between our work and the existing tree-structured approaches are that (1) SAN integrates syntax constraints representation into deep neural network feature learning.  (2) Our method is a holistic syntax-aware approach that accurately identifies and locates components of MEs with complex structural relationships. As shown in Fig. \ref{bad cases}, SAN locates and recognizes the given MEs correctly while DWAP-TD misses a component of MEs. (3) SAN minimizes high computational costs by parsing one component to another instead of the individual parent and child nodes.
%2) The difficulty of HMER mostly relies on considering structural complexity rather than symbol recognition. However, these methods focus on the individual prediction of a parent node and a child node to generate a new symbol instead of a holistic syntax-aware approach.
%Our model extends the tree-based decoder by explicitly following grammatical production rules in the decoding process, while in \cite{zhang2020tree}, expression was separated into parent-child node pairs, which weakens the learning of inherent language structure. Except that, using explicit grammar avoids redundant computation and obtains efficient inference. 
%To solve these challenges above, we propose a method, which firstly incorporate syntax information into the encoder-decoder network. In this way, our proposed model can effectively describe the syntax context of expressions, avoiding the structure prediction errors of HMER.
%(4) Besides generating meaningful formulas of components, our method has more potential to support partial expression retrieval and similar tasks with complex structural relationships.

%Therefore, SAN has the holistic representation of syntax constraint in deep neural network feature learning and can robustly describe the syntax context of expressions, with faster inference time than its prior arts.

%To solve these challenges, we proposed a neural network architecture equipped with syntactic rules that efficiently divides a syntax tree into different components to avoid errors caused by tree structure ambiguity. The proposed method learns the grammatical relationship between the structures based on the syntactic rules and navigates the grammar tree to create components according to the structural relationship. Unlike the existing tree-structured approaches, (1) SAN integrates syntax information into deep network feature learning.  (2) Besides the effectiveness in recognition, our method accurately identifies and locates components of MEs with complex structural relationships. As shown in Fig. \ref{bad cases} a and b, SAN locates and recognizes the given MEs correctly while DenseWAP-TD misses to locate and accurately predict. (3) SAN minimizes high computational costs by parsing one component to another instead of the individual parent and child nodes. (4) Besides generating meaningful formulas of components, our method has more potential to support partial expression retrieval and similar tasks with complex structural relationships.In this way, our proposed model can robustly describe the syntax context of expressions, avoiding the structure prediction errors of HMER with faster inference time.

%To solve these challenges, we propose a syntax-aware network that incorporates syntax information into the encoder-decoder network and efficiently divides a syntax tree into different components to avoid errors caused by tree structure ambiguity. In this way, our proposed model can effectively describe the syntax context of expressions, avoiding the structure prediction errors of HMER with faster inference time.
